Sequential Movie Genre Prediction using Average Transition Probability with Clustering

In recent movie recommendations, predicting the user's sequential behavior and suggesting the next movie to watch is one of the most important issues. However, capturing such sequential behavior is not easy because each user's short-term or long-term behavior must be taken into account. For this reason, many research results show that the performance of recommending a specific movie is not very high in a sequential recommendation. In this paper, we propose a cluster-based method for classifying users with similar movie purchase patterns and a movie genre prediction algorithm rather than the movie itself considering their short-term and long-term behaviors. The movie genre prediction does not recommend a specific movie, but it predicts the genre for the next movie to watch in consideration of each user's preference for the movie genre based on the genre included in the movie. Through this, it is possible to provide appropriate guidelines for recommending movies including the genre to users who tend to prefer a specific genre. In particular, in this paper, users with similar genre preferences are organized into clusters to recommend genres, and in clusters that do not have relatively specific tendencies, genre prediction is performed by appropriately trimming genres that are not necessary for recommendation in order to improve performance. We evaluate our method on well-known movie datasets, and qualitatively that it captures personalized dynamics and is able to make meaningful recommendations.

==> mymath.tex <==
%%%%%%%%%%%% real, integer notation
\newcommand{\real}{{\mathbb R}}
\newcommand{\integer}{{\mathbb Z}}


% boldface characters
% macro by mung


\newcommand{\td}{\ensuremath{t_{\text{dl}}}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bbx}{\ensuremath{{\bm x}}}
\newcommand{\bbc}{\ensuremath{{\bm c}}}
\newcommand{\bu}{\ensuremath{{\bm u}}}

\newcommand{\bz}{\ensuremath{{\bm z}}}
\newcommand{\ba}{\ensuremath{{\bm a}}}
\newcommand{\be}{\ensuremath{{\bm e}}}
\newcommand{\br}{\ensuremath{{\bm r}}}
\newcommand{\by}{\ensuremath{{\bm y}}}
\newcommand{\bby}{\ensuremath{{\bm y}}}
\newcommand{\bbq}{\ensuremath{{\bm q}}}


\newcommand{\bp}{\ensuremath{{\bm p}}}
\newcommand{\bh}{\ensuremath{{\bm h}}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bA}{\ensuremath{{\bm A}}}

\newcommand{\bF}{\bm{F}}
\newcommand{\bN}{\ensuremath{{\bm N}}}
\newcommand{\bbf}{\ensuremath{{\bm f}}}
\newcommand{\bG}{\ensuremath{{\bm G}}}
\newcommand{\bQ}{\ensuremath{{\bm Q}}}
\newcommand{\bH}{\ensuremath{{\bm H}}}
\newcommand{\bW}{\ensuremath{{\bm W}}}
\newcommand{\bJ}{\ensuremath{{\bm J}}}
\newcommand{\bg}{\ensuremath{{\bm g}}}
\newcommand{\bs}{\ensuremath{{\bm s}}}

\newcommand{\bbv}{\ensuremath{{\bm v}}}
\newcommand{\bbz}{\ensuremath{{\bm z}}}
\newcommand{\bbu}{\ensuremath{{\bm u}}}
\newcommand{\bbm}{\ensuremath{{\bm m}}}
\newcommand{\bbU}{\ensuremath{{\bm U}}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bbr}{\ensuremath{{\bm r}}}
\newcommand{\bbalpha}{\ensuremath{{\bm \alpha}}}
\newcommand{\brho}{\ensuremath{{\bm \rho}}}


% \newcommand{\bblambda}{\mbox{\boldmath \ensuremath{\lambda}}}
% \newcommand{\blambda}{\mbox{\boldmath \ensuremath{\lambda}}}

% \newcommand{\bmu}{\mbox{\boldmath \ensuremath{\mu}}}
% %\newcommand{\bmu}{\mu}

% \newcommand{\bbeta}{\mbox{\boldmath \ensuremath{\beta}}}
% \newcommand{\btheta}{\mbox{\boldmath \ensuremath{\theta}}}
% \newcommand{\bv}{\ensuremath{{\mathbf v}}}
% %\newcommand{\reals}{\ensuremath{\mathbf{R}}}
\newcommand{\bR}{\bm{R}}
% \newcommand{\bw}{\ensuremath{{\mathbf w}}}
% % \newcommand{\bF}{F}


%%%%%%%%%%%% Sets, calligraphic characters...
\newcommand{\cR}{\ensuremath{\mathcal R}}
\newcommand{\set}[1]{\ensuremath{\mathcal #1}}
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}

\newcommand{\node}[1]{\ensuremath{{\tt #1}}}
\newcommand{\nn}[1]{\node{#1}}

\newcommand{\singleq}[1]{\text{`}#1\text{'}}

\newcommand{\mytitle}[1]{\medskip \noindent{\em #1} \smallskip}
\newcommand{\mytitlehead}[1]{\noindent{\em #1} \smallskip}

\newcommand{\separator}{
  \begin{center}
    \rule{\columnwidth}{0.3mm}
  \end{center}
}
\newenvironment{separation}{ \vspace{-0.3cm}  \separator  \vspace{-0.2cm}}
{  \vspace{-0.4cm}  \separator  \vspace{-0.1cm}}

%%%%%%%%%%%%%%%% other macros %%%%%%%%%%%%%%%%%%
\def\un{\underline}
\def\ov{\overline}
\def\Bl{\Bigl}
\def\Br{\Bigr}
% \def\bl{\bigl}
% \def\br{\bigr}
\def\lf{\left}
\def\ri{\right}
\def\st{\star}

\def\eg{{\it e.g.}}
\def\ie{{\it i.e.}}

%\newcommand{\eqdef}{{\triangleq}}

% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{property}{Property}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
% \newtheorem{algorithm}{Algorithm}[section]
\newtheorem{condition}{Condition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{problem}{Problem}[section]

\newcommand{\bprob}[1]{\mathbb{P}\Bl[ #1 \Br]}
\newcommand{\prob}[1]{\mathbb{P}[ #1 ]}
\newcommand{\expect}[1]{\mathbb{E}[ #1 ]}
\newcommand{\bexpect}[1]{\mathbb{E}\Bl[ #1 \Br]}
\newcommand{\bbexpect}[1]{\mathbb{E}\lf[ #1 \ri]}
\newcommand{\vari}[1]{\text{VAR}[ #1 ]}
\newcommand{\bvari}[1]{\text{VAR}\Bl[ #1 \Br]}


\newcommand{\exming}{\ensuremath{\text{ExMin}_g} }
\newcommand{\imp}{\Longrightarrow}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bemn}{\begin{multiline}}
\newcommand{\eemn}{\end{multiline}}

\newcommand{\sqeq}{\addtolength{\thinmuskip}{-4mu}
\addtolength{\medmuskip}{-4mu}\addtolength{\thickmuskip}{-4mu}}

\newcommand{\unsqeq}{\addtolength{\thinmuskip}{+4mu}
\addtolength{\medmuskip}{+4mu}\addtolength{\thickmuskip}{+4mu}}

% floor function
\newcommand{\lfl}{{\lfloor}}
\newcommand{\rfl}{{\rfloor}}
\newcommand{\floor}[1]{{\lfloor #1 \rfloor}}

\newcommand{\grad}[1]{\nabla #1}

% \newcommand{\sqeq}{\addtolength{\thinmuskip}{-4mu}
%   \addtolength{\medmuskip}{-4mu}\addtolength{\thickmuskip}{-4mu}}
% \newcommand{\unsqeq}{\addtolength{\thinmuskip}{+4mu}
%   \addtolength{\medmuskip}{+4mu}\addtolength{\thickmuskip}{+4mu}}

% \newcommand{\bea}{\begin{eqnarray}}
%   \newcommand{\eea}{\end{eqnarray}}
% \newcommand{\beas}{\begin{eqnarray*}}
%   \newcommand{\eeas}{\end{eqnarray*}}
% \newcommand{\bd}{\begin{displaymath}}
%   \newcommand{\ed}{\end{displaymath}}
% \newcommand{\be}{\begin{equation}}
%   \newcommand{\ee}{\end{equation}}
% \newcommand{\vs}{\vspace{0.2in}}
% \newcommand{\hs}{\hspace{0.5in}}
% \newcommand{\el}{\end{flushleft}}
% \newcommand{\bl}{\begin{flushleft}}
% \newcommand{\bc}{\begin{center}}
% \newcommand{\ec}{\end{center}}
% \newcommand{\remove}[1]{}

% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{prop}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{defi}{Definition}
% \newtheorem{assum}{Assumption}
% \newtheorem{example}{Example}
% \newtheorem{property}{Property}
% \newtheorem{remark}{Remark}

% \newcommand{\separator}{
%   \begin{center}
%     \rule{\columnwidth}{0.3mm}
%   \end{center}
% }

% \newenvironment{separation}
% { \vspace{-0.3cm}
%   \separator
%   \vspace{-0.25cm}
% }
% {
%   \vspace{-0.5cm}
%   \separator
%   \vspace{-0.15cm}
% }

% \renewcommand{\baselinestretch}{0.98}

\def\A{\mathcal A}
\def\oA{\overline{\mathcal A}}
\def\S{\mathcal S}
\def\D{\mathcal D}
\def\eff{{\rm Eff}}

\def\cU{{\cal U}}
\def\cM{{\cal M}}
\def\cV{{\cal V}}
\def\cA{{\cal A}}
\def\cX{{\cal X}}
\def\cN{{\cal N}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cI{{\cal I}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
\def\cC{{\cal C}}
\def\cR{{\cal R}}
\def\id{{\rm Id}}
\def\st{{\rm st}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\N{\mathbb{N}}
\def\R{\mathbb{R}}
\def\cB{{\cal B}}
\def\cP{{\cal P}}
\def\cS{{\cal S}}
%\def\and{\quad\mbox{and}\quad}
\def\ind{{\bf 1}}

\def\bmg{{\bm{\gamma}}}
\def\bmr{{\bm{\rho}}}
\def\bmq{{\bm{q}}}
\def\bmt{{\bm{\tau}}}
\def\bmn{{\bm{n}}}
\def\bmcapn{{\bm{N}}}
\def\bmrho{{\bm{\rho}}}

\def\igam{\underline{\gamma}(\lambda)}
\def\sgam{\overline{\gamma}(\lambda)}


\def\PP{{\mathrm P}}
\def\EE{{\mathrm E}}
\def\iskip{{\vskip -0.4cm}}
\def\siskip{{\vskip -0.2cm}}

\def\bp{\noindent{\it Proof.}\ }
\def\ep{\hfill $\Box$}


% \newcommand{\set}[1]{\mathcal{#1}}




